Edge-Disjoint Spanning Trees on Star-Product Networks

A star-product operation may be used to create large graphs from smaller factor graphs. Network topologies based on star-products demonstrate several advantages including low-diameter, high scalability, modularity and others. Many state-of-the-art diameter-2 and -3 topologies~(Slim Fly, Bundlefly, PolarStar etc.) can be represented as star products. In this paper, we explore constructions of edge-disjoint spanning trees~(EDSTs) in star-product topologies. EDSTs expose multiple parallel disjoint pathways in the network and can be leveraged to accelerate collective communication, enhance fault tolerance and network recovery, and manage congestion. Our EDSTs have provably maximum or near-maximum cardinality which amplifies their benefits. We further analyze their depths and show that for one of our constructions, all trees have order of the depth of the EDSTs of the factor graphs, and for all other constructions, a large subset of the trees have that depth.

==> maximality.tex <==
\lmedit{
\subsection{Old Upper bounds }
We return to the question of maximum cardinality of sets of EDSTs. Lemma~\ref{lemma:sptree_identity} gives a general upper bound in terms of the number of edges and vertices of the star product. We give here other bounds, this time in terms of the theoretical maximum number of EDSTs that may be constructed in each of the factor graphs.
\begin{lemma}\label{lemma_max_bounds}
    Let $G = G_s*G_n$ be a star product, with $G$ simple. Let $t_s$ and $t_n$ be some number of EDSTs of $G_s$ and $G_n$, and let $r_s$ and $r_n$ be the number of unused edges in $G_s$ and $G_n$ when the $t_s$ and $t_n$ EDSTs are constructed. Then 
    $$
    t_s+t_n+\floor{\frac{r_s-t_s}{|V_s|} +\frac{r_n-t_n}{|V_n|} +\frac{1}{2}}
    $$
    is the largest number of EDSTs that may be constructed in $G$.
\end{lemma}
\begin{proof}
    We have from Theorem~\ref{th:star_props} that
    \begin{align*}
        |E_G| &= |E_s| |V_n|+|E_n| |V_s| \text{ and }\\
        |V_G| &= |V_s| |V_n|,
    \end{align*}
    and we know that
    \begin{align*}
        |E_s| &= t_s(|V_s|-1)+r_s \text{ and }\\
        |E_n| &= t_n(|V_n|-1)+r_n.
    \end{align*}
    From Equation~\ref{eq:edsts}, we have that
    \begin{align*}
        t = \floor{\frac{|E_G|}{|V_G|-1}} 
        &= \floor{\frac{|E_G|}{|V_G|} + \frac{|E_G|}{|V_G|(|V_G|-1)}}\\
        &\le \floor{\frac{|E_G|}{|V_G|} + \frac{1}{2}} \\
        &= \floor{\frac{|E_s| |V_n|+|E_n| |V_s|}{|V_s| |V_n|} + \frac{1}{2}}\\
        &= \floor{\frac{|E_s|}{|V_s|} + \frac{|E_n|}{|V_n|} + \frac{1}{2}}\\
        &=t_s+t_n+\floor{\frac{r_s-t_s}{|V_s|} +\frac{r_n-t_n}{|V_n|} +\frac{1}{2}}.
    \end{align*}
\end{proof}
\begin{corollary}\label{cor_max_bounds}
    Let $G = G_s*G_n$ be a star product, with $G$ simple. Let $T_s$ and $T_n$ be the maximum number of EDSTs of $G_s$ and $G_n$ that can be constructed, and let $R_s$ and $R_n$ be the number of unused edges in $G_s$ and $G_n$ if the $T_s$ and $T_n$ EDSTs are constructed. Let
    $$
    T = \begin{cases*}
            T_s+T_n, &\text{if $R_s = T_s$ and $R_n = T_n$}, \\
            T_s+T_n+2, &\text{if $R_s \ge T_s$ and $R_n \ge T_n$},\\ 
            T_s+T_n+1, &\text{if $R_s \ge T_s$ or $R_n \ge T_n$},\\ 
            T_s+T_n, &\text{if $R_s < T_s$ and $R_n < T_n$}. 
        \end{cases*} 
    $$
    Then $T$ is an upper bound on the number of EDSTs that can be constructed in $G$. 
\end{corollary}
\begin{proof}
    We have that 
    \begin{align*}
        |E_s| &= T_s(|V_s|-1)+R_s \text{ and }\\
        |E_n| &= T_n(|V_n|-1)+R_n,
    \end{align*}where 
    \begin{align*}
        |R_s| &< |V_s|-1  \text{ and }\\
        |R_n| &< |V_n|-1 ,
    \end{align*}
    since $T_s$ and $T_n$ are the maximum number of EDSTs that can be constructed in $G_s$ and $G_n$. The corollary then follows directly from Lemma~\ref{lemma_max_bounds}.
\end{proof}
\begin{theorem}
    Let $G = G_s*G_n$ be a star product, with $G$ simple, and let the number of EDSTs in $G_s$ and $G_n$ be $T_s$ and $T_n$, where $T_s$ and $T_n$ have the maximum cardinality possible. 
    
    Then the EDST constructions in this paper have cardinality within $2$ of the theoretical maximum for $G$.
\end{theorem}
\begin{proof}
    Let $T$ be the number of EDSTs constructed using the methods in this paper producing the most EDSTs for given conditions on $r_s$, $r_n$, $t_s$ and $t_n$. Then
    $$
    T = \begin{cases*}
            T_s+T_n, &\text{if $R_s = T_s$ and $R_n = T_n$}, \\
            T_s+T_n, &\text{if $R_s \ge T_s$ and $R_n \ge T_n$},\\ 
            T_s+T_n-1, &\text{if $R_s \ge T_s$ or $R_n \ge T_n$},\\ 
            T_s+T_n-1, &\text{if $R_s < T_s$ and $R_n < T_n$, Prop.~\ref{property:no_edge_conditions}},\\
            T_s+T_n-2, &\text{otherwise}, 
        \end{cases*} 
    $$
by Theorem~\ref{th:r_eq_t}, Corollaries~\ref{cor:r_ge_t} and \ref{cor:t_r_ge_or}, and Theorems~\ref{th:t_r_lt} and \ref{th:t_r_generic}, as displayed in Table~\ref{tab:star_ths}. The theorem then follows by direct comparison to Corollary~\ref{cor_max_bounds}.
\end{proof}
}

==> new_lemma.tex <==
The bounds in Proposition~\ref{prop:max_bounds_tr} are less strict than the above bounds,
but instead establish a linear relationship between the maximum number of EDSTs in
the product and 
in the factors. 
They are used in Theorem~\ref{th:one_less_than_max} to show that our constructions are \lmedit{within $1$ of} maximum size, in Theorem~\ref{th:r_eq_t} to show maximum cardinality when \lmedit{$r_i = t_i$, and in Theorem~\ref{th:t_r_lt} to show maximum cardinality when $r_s < t_s$ and $r_n < t_n$}. 

\begin{restatable}[]{proposition_restate}{maxboundstr}
\label{prop:max_bounds_tr}\footnote{\lmedit{Proposition~\ref{prop:max_bounds_tr} gives bounds that tighten those we presented in \cite{edst_ipdps_2025} by $1$, except for the $\rho_i=\tau_i$ case, which stays the same.}}
    Let $G^* = G_s*G_n$ be a star product, with $G^*$ simple. Let \lmedit{$\tau_s$ and $\tau_n$ be the canonical upper bounds on} the number of EDSTs in $G_s$ and $G_n$, and let $\rho_s$ and $\rho_n$ be the number of unused edges that would be in $G_s$ and $G_n$ if the $\tau_s$ and $\tau_n$ EDSTs were constructed. Then \lmedit{an upper bound $\tau$ on the number of EDSTs in $G^*$ that may be produced} is
    $$
    \tau = 
        \begin{cases*}
            \tau_s+\tau_n+1, &\text{if $\rho_s \ge \tau_s$ and $\rho_n \ge \tau_n$},\\ 
            \tau_s+\tau_n, &\text{if $\rho_s = \tau_s$ and $\rho_n = \tau_n$}, \\
            \tau_s+\tau_n, &\text{if $\rho_s \ge \tau_s$ or $\rho_n \ge \tau_n$ (but not both)},\\ 
            \tau_s+\tau_n-1, &\text{if $\rho_s < \tau_s$ and $\rho_n < \tau_n$}.
        \end{cases*} 
    $$ 
\end{restatable}
\begin{proof}
    The proof is given in Appendix~\ref{sec:appendix_proofs}.
\end{proof}


==> table_star_ths_depth.tex <==
\begin{table*}[!ht]
\renewcommand\arraystretch{1.5}
\centering
\footnotesize
\noindent\adjustbox{max width=\textwidth}
{
\begin{tabular}{|l|l|l|l|l|l|l|l|}
\hline
\rowcolor[HTML]{EFEFEF} 
\textbf{Conditions}  & \textbf{EDSTs} & \textbf{Max?} & \textbf{EDST Thm.} &\textbf{Max Depth} &\textbf{Min Depth} 
&\textbf{\begin{tabular}[c]{@{}c@{}}\# Min-Depth \\EDSTs \end{tabular}}
&\textbf{Depth Thms.} \\
\hline
\begin{tabular}[c]{@{}l@{}}$r_s=t_s$ AND $r_n=t_n$\end{tabular} & $t_s+ t_n$ & Yes & \ref{th:r_eq_t} & $(d_{s_1}+1)(2d_{n_1} + 2r_s) + d_{s_1}$ & $2d_{s_i} + d_{n_1}$&$t_s-1$ &\ref{thm:depth_maximum}, \ref{cor:depth_maximum}\\ \hline
\begin{tabular}[c]{@{}l@{}}$r_s\ge t_s$ AND $r_n\ge t_n$\end{tabular} & $t_s+ t_n$ & Maybe & \ref{cor:r_ge_t} &  $(d_{s_1}+1)(2d_{n_1} + 2r_s) + d_{s_1}$& $2d_{s_i} + d_{n_1}$ & $t_s-1$&\ref{thm:depth_maximum}, \ref{cor:depth_maximum} \\ \hline
\begin{tabular}[c]{@{}l@{}}$r_s\ge t_s$ OR $r_n\ge t_n$\end{tabular} & $t_s+ t_n-1$ & Maybe & \ref{cor:t_r_ge_or} &  $(d_{s_1}+1)(2d_{n_1} + 2r_s) + d_{s_1}$& $2d_{s_i} + d_{n_1}$& $t_s-1$&\ref{thm:depth_maximum}, \ref{cor:depth_maximum}\\ \hline
\begin{tabular}[c]{@{}l@{}}\end{tabular}Any star product (Universal) & $t_s+ t_n-2$ & Maybe & \ref{th:t_r_generic} 
& $\max(2d_{s_i} + d_{n_1},d_{s_1} + 2d_{n_i})$ 
& $\min(2d_{s_i} + d_{n_1},d_{s_1} + 2d_{n_i})$ &$t_s-1$ or $t_n-1$&\ref{thm:depth_universal_1}, \ref{thm:depth_universal_2}\\ \hline
\end{tabular}
}
\caption{The number of EDSTs that are constructed on star products with connected factor graphs, given conditions on $t_i$, the number of EDSTs of factor $G_i$, and $r_i$, the number of remaining edges in $G_i$ that are not in any EDST. Here, $d_{s_i}$ and $d_{n_i}$ are the depth of the $i^{th}$ EDST used from the structure graph $G_s$ and supernode $G_n$, respectively. The Universal construction, which applies to any star product, gives a set of trees, all of which have depth linear in the depths of the EDSTs of $G_s$ and $G_n$. Other constructions have conditions on the factor graphs and give $1$ or $2$ extra trees, with some constructions reaching maximum cardinality. Although their worst-case depths are quadratic in the depths of the EDSTs of $G_s$ and $G_n$, these constructions still have a large subset of small depth trees. A comparison of the merits of different solutions is discussed in Section~\ref{sec:discussion}. 
\vspace{-.15in}}
\label{table:star_ths}
\end{table*}


